A Typology of Decision-Making Tasks for Visualization

Despite decision-making being a vital goal of data visualization, little work has been done to differentiate decision-making tasks within the field. While visualization task taxonomies and typologies exist, they often focus on more granular analytical tasks that are too low-level to describe large complex decisions, which can make it difficult to reason about and design decision-support tools. In this paper, we contribute a typology of decision-making tasks that were iteratively refined from a list of design goals distilled from a literature review. Our typology is concise and consists of only three tasks: CHOOSE, ACTIVATE, and CREATE. Although decision types originating in other disciplines exist, we provide definitions for these tasks that are suitable for the visualization community. Our proposed typology offers two benefits. First, the ability to compose and hierarchically organize the tasks enables flexible and clear descriptions of decisions with varying levels of complexities. Second, the typology encourages productive discourse between visualization designers and domain experts by abstracting the intricacies of data, thereby promoting clarity and rigorous analysis of decision-making processes. We demonstrate the benefits of our typology through four case studies, and present an evaluation of the typology from semi-structured interviews with experienced members of the visualization community who have contributed to developing or publishing decision support systems for domain experts. Our interviewees used our typology to delineate the decision-making processes supported by their systems, demonstrating its descriptive capacity and effectiveness. Finally, we present preliminary findings on the usefulness of our typology for visualization design.

==> tex/Discussion.tex <==
\section{Discussion \kami{leave for the end, we have a lot of discussions throughout the paper}}
\label{sec:discussion}
%The flexibility of the evaluation functions, especially in the CHOOSE and ACTIVATE tasks, allows for judgement that is consistently or inconsistently applied [citation].
%In other words, cognitive biases are on an orthogonal axis of these task definitions.

The evaluation of our decision-making task typology received predominantly positive feedback from the participants in our interview study. 
In this section, we analyze additional feedback from participants to identify potential areas for future research.
%discuss
%some of the other comments made by the participants and discuss potential avenues for future research based on their feedback.



\subsection{Measuring the Effectiveness of the Typology}
%Measuring the effectiveness of a taxonomy or a typology is difficult.
In addition to conducting an interview study with visualization researchers to evaluate our typology, we also assess its effectiveness according to the criteria established by Brehemer et al.\cite{brehmer_multi-level_2013} and Yi et al.\cite{yi2007toward}. 
Specifically, we examine our typology through the lens of three dimensions proposed by Beaudouin-Lafon\cite{beaudouin2004designing}: (1) \textit{descriptive power}: ``the ability to describe a significant range of existing [designs]'', (2) \textit{evaluative power}: ``the ability to help assess multiple design alternatives'', and (3) \textit{generative power}: ``the ability to help designers create new designs.''

\kami{R3 said that this part is redundant, see R3, question 5}
We have showcased the descriptive capabilities of our typology through four case studies and an interview study. 
In each instance, designers successfully utilized our typology to construct diagrams that effectively described their decision-making problems. 
Furthermore, we have begun to demonstrate how the typology could facilitate the evaluation and the identification of similar decision problems. 
Our case studies illustrated the potential of using these diagrams to compare the similarities and differences between domain-specific decision problems in a domain-agnostic way.

Finally, we assess the generative aspect of our typology using the definition provided by Brehmer et al.\cite{brehmer_multi-level_2013}. 
Specifically, a typology is generative if has a systematic approach for using it to create workflows or diagrams. 
Our proposed hierarchical decomposition process of decision tasks corresponds with this definition. 
Starting from the root level, participants demonstrated the ability to recursively expand each node into a composed set of decision tasks, culminating in the creation of a complete diagram. 
This approach allows visualization designers to methodically externalize decision problems in a structured manner, facilitating a gradual but precise representation of the decision-making process.


% \subsection{From Typology to Visualization Design \kami{Should we remove this subsection? maybe add this to future work?}}

% % \subsubsection{Quotes and topics from initial interviews}
% % \noindent \textbf{}

% %In addition to utilizing our typology to describe decision-making problems, we see another potential application.
% Some participants in our study highlighted the opportunity to integrate the diagrams created using our typology with visualization designs. 
% By pairing these diagrams with their associated visualization designs, it becomes feasible to explore these relationships to develop recommendation systems of decision-support tools, following a similar approach as the Draco system\cite{moritz2018formalizing}. For instance, the Homefinder Revisited case study, as described in Section~\ref{subsec:homefinder}, illustrates a simple diagram representing a multi-criteria decision-making (MCDM) problem. 
% Due to the widespread use of MCDM, this motif occurs in many other, more intricate decision-making scenarios. 
% In the Umbra and Centaurus case studies illustrated in Figures~\ref{fig:umbra} and~\ref{fig:centaurus}, the same MCDM motif is evident (observed in the top three nodes), indicating that MCDM is a component of both the Umbra and Centaurus decision problems as well.
% When paired with their associated visualization designs, we can begin to identify and extract visualization design patterns that represent MCDM or other similar sub-decision tasks.
% In our future work, we aim to investigate how we can integrate our typology diagrams with visualization design processes to assist designers of decision-support tools.


==> tex/Reviews.tex <==
\section{Reviews}
\subsection{Reviewer 2}
The connection of Sections 3 and 4 must be improved; it must become more clear how much inspiration from \cite{fischhoff_communicating_2014, fischhoff2020judgment} was taken and how much is new; further, it must become more clear how the three tasks forming the base of the typology were derived from the analyzed work; in addition, in the description of the tasks in section 4, all the analysis of the papers collected by \cite{oral_information_2023, shi_how_2023} that are supposed to be the base are never mentioned again.



In the Fishoff paper \cite{fischhoff_communicating_2014} the tasks are loosely described and the focus is on identifying uncertainty and how to mitigate it rather than formalizing the definitions of the decision tasks. In the list of decision types they present, we include what are the things that we kept/extended for each decision:

a) Decisions about action thresholds: Is it time to act? 
Decisions about action thresholds involve determining when to act based on evidence surpassing a predefined threshold. We think that this type of task can be extended with thresholds other than temporal, thus forming the base of our ACTIVATE task.

b) Decisions with fixed options: Which is best?
Decisions with fixed options involve choosing the best option among a set. This classic task is mentioned in the CHOICE stage of Simon’s decision-making phases \cite{simon1960new,campitelli2010herbert}, so we started adding more nuance on top of this base task until we got the CHOICE task.

c) Decisions about potential options: What is possible?
Decisions about potential options involve creating new options rather than waiting for a signal or choosing from fixed ones. This one is again mentioned as a preparatory task in Simon's work \cite{simon1960new,campitelli2010herbert}, so it’s a good starting point for the CREATE task in our typology.

While these are good bases from which to start expanding our set of decision-making tasks, they are not enough. When we want to analyze decision-making in visual analytics, we need to know what the inputs and outputs of these decisions are, what happens when a decision task is performed, and how these decisions interact with each other (see design goals section).

Dimara’s “A task-based taxonomy of cognitive biases for information visualization” \cite{dimara2018task} presents a taxonomy with the following task-categories: estimation, decision, hypothesis assessment, causal attribution, recall, opinion, and other. Note that there is just one general ‘DECISION’ task. While this is useful for finding biases in visual analytics, it is not useful for effectively describing how people make decisions, let alone how to generate new designs. Plus, this taxonomy was extracted from experiments where bias was measured, a type of evaluation that is barely ever used to evaluate visual analytics tools and decision support systems in the visualization community.

Padilla’s \cite{padilla_decision_2018} focuses on the process of decision making with visualizations by outlining a dual-process model. The first mechanism in this model produces fast and intuitive decisions, while the second one facilitates more slower more effortful decisions with visualizations. While this informed our typology that focusing on the process of decision making is relevant, it doesn’t provide us on how to describe such processes, nor how different types of decisions interact with this dual-process model. Takemura \cite{takemura2021behavioral} emphasizes that decision strategies vastly differ based on the task, task dependence, and even number of alternatives \cite{takemura2021behavioral, bettman1979information, payne1991consumer, takemura1993protocol}. Thus, unless we understand these aspects in visual analytics, it would be hard to reason efficiently on what the biases are in visual analytics with the end goal of creating efficient decision support tools.

\cite{wang2007cognitive} Only addresses the CHOICE task. Nevertheless, it presents an interesting perspective on the definition of decision making, where it says that decision making is about the construction of the decision criteria (or functions) and strategies to use them to make the decision. Thus, this prompted us to think about what kind of evaluation is happening behind the scenes of each type of decision, and how they interact with the inputs and outputs. <Explain further?>



==> tex/SupplementalMaterials.tex <==
\newpage

\section{Supplemental Materials}
\label{sec:supplementals}
\subsection{Quotes Supporting the Design Goals for a Decision Task Typology}
%[itemsep=0pt, parsep=3pt, leftmargin=*]
\begin{enumerate}[label=\textbf{G\arabic*}]
    \item \label{goal:iteration} \textbf{Iteration}: Given that decision-making processes in visualization often involve cycles and iterations, our typology should incorporate a mechanism to express such iterative patterns.
    \begin{itemize}[leftmargin=*]
        \item ``\textit{By working with the domain experts, we constructed a three-stage iterative workflow for analyzing and improving bus networks}''\cite{weng2021towardsbetterbus}
        \item ``\textit{Planners, stakeholders, and development team members work together in planning their project using ReleasePlanner; the iterative standard planning procedures include...}''\cite{aseniero2015stratos}
    \end{itemize}
    \item \label{goal:hierarchical} \textbf{Hierarchical structure}: Decisions are intricate and can be deconstructed into subtasks, necessitating the ability of our typology to capture these hierarchical relationships.
    \begin{itemize}[leftmargin=*]
        \item ``\textit{Our final design improved the layout and probability encoding of the hierarchical-oriented choices.}''\cite{guo2019uncertaintyandalternatives}
        \item ``\textit{We present two design lessons we have learned while developing BNVA. First, hierarchical exploration is mandatory for complex data like bus networks. [...] In this study, we employed a hierarchical exploration approach to dissect a network with multiple coordinated views from the overview to the details and provide visual hints for the users to drill down in the dataset and find interesting patterns.}''\cite{weng2021towardsbetterbus}
    \end{itemize}
    \item \label{goal:process-centric} \textbf{Process-centric approach}: Our typology should focus on delineating the sequence of decisions users encounter, rather than merely representing data-processing flow or interaction order typically outlined in task lists and design requirements of application papers and design studies.
    \begin{itemize}[leftmargin=*]
        \item ``\textit{Using a laboratory model, the authors have investigated various possible methods for breach closure, utilizing procedures such as single-and multi-barrier embankments with different ways of positioning sandbags. [...] We have identified 7 major phases that led to the final solution.}''\cite{waser2010worldlines}
        \item ``\textit{...capturing metadata of the visual exploration process is a key component of the analysis process. Our history tree visualization is able to record users’ decisions and allow them to compare, modify and insert new decisions.}''\cite{afzal2011decisionsupportforepidemic}
        \item ``\textit{Our approach aims to implement the scenario pool concept as we see it: first, create many plans in the preparation phase; second, quickly pick the most appropriate one in the response phase.}''\cite{waser2014manyplans}
        
    \end{itemize}
    \item \label{goal:data-flexibility} \textbf{Information Processing-Focused}: The decision tasks within our typology should demonstrate flexibility and impartiality towards input and output types, instead emphasizing how information is processed and evaluated.
    \begin{itemize}[leftmargin=*]
         \item ``\textit{The person in charge  [..] %of the defenses 
         has an overview of an area where a disaster can happen, and a number of protection measures available. [...] %Given that there is only a limited amount of time, materials and personnel that can be used, the selection of the measures to be deployed is a difficult task. 
         The goal of our steering environment is to allow the user to experiment with various options, and to do it as intuitively as possible.}''\cite{ribicic2012sketchinguncertainty}
         %\item ``\textit{We have experimented [...] %with this approach 
         %in the area of travel planning and developed a system called SmartClient Travel[...].% which supports this process.It includes tools for need identification, visualization of alternatives, and choosing the most suitable one. [...] The catalog should propose solutions and compare them to alternatives, and thus elicit refinement of the buyer's specifications.}'' \cite{pu2000smartclient}
         \item ``\textit{...only information on a few products is given to the buyers, leaving them wondering what other alternatives are available.}''\cite{weng2018homefinder}
          \item ``\textit{This interactive exploratory tool helps the casual decision-maker quickly choose between various financial portfolio options and view possible outcomes.}''\cite{rudolph2009finvis}
    \end{itemize}
\end{enumerate}

\subsection{Diagrams Created by Our Participants}.
\begin{figure}[ht!]
\centering
  \includegraphics[width=0.9\linewidth]{figs/hierarchy_annotation.pdf}
  \caption{A hierarchy annotation used by one of the participants during the interview study. In this figure, the triangles (and the arrows) indicate the role of a decision-maker in an organization's hierarchy.
  }
  \label{fig:annotation}
\end{figure}

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\textwidth]{figs/interview_diagrams.pdf}
    \caption{Diagrams created by our participants during the interview study. Texts, labels, and annotations that contain identifiable information have been removed to preserve anonymity. We labeled the diagrams with the domain of application.}
    \label{fig:collage}
\end{figure*}
